The Dark Side: Security Concerns in Machine Learning for EDA

The growing IC complexity has led to a compelling need for design efficiency improvement through new electronic design automation (EDA) methodologies. In recent years, many unprecedented efficient EDA methods have been enabled by machine learning (ML) techniques. While ML demonstrates its great potential in circuit design, however, the dark side about security problems, is seldomly discussed. This paper gives a comprehensive and impartial summary of all security concerns we have observed in ML for EDA. Many of them are hidden or neglected by practitioners in this field. In this paper, we first provide our taxonomy to define four major types of security concerns, then we analyze different application scenarios and special properties in ML for EDA. After that, we present our detailed analysis of each security concern with experiments.

==> _txt/EDA.tex <==



\section{The Impact on EDA Software}
\label{sec:2}


\subsection{Security Challenges on EDA Software}

When discussing the security challenges of EDA software in this paper, we do not emphasize traditional malicious software attacks like virus, malware, or spyware. Instead, we focus on the increasingly serious threat from ML algorithms, most of which are trained to learn the functionality of EDA tools and then can be applied to partially or even entirely replace these tools in circuit design flow. 


This is a quite unique threat from ML applications. Different from most ML applications where ML models are applied to replace human efforts, ML for EDA methods have been applied to accomplish the tasks of both human designers and EDA tools. While the impact of ML on employment has been extensively discussed, the impact on commercial software like EDA tools is more complex and much less studied. This will greatly benefit design companies by reducing overall turn-around time and improving chip quality, but will be a double-edged sword for EDA companies. On one hand, traditional EDA companies can improve their tools with ML models. On the other hand, other developers or design teams may build their own ML models based on the state-of-the-art EDA tools. They may even further open-source these models or sell them by license or as a service. Since these ML models are developed based on EDA tools, they are strong competitors of traditional tools on the EDA market.  


Although EDA vendors have widened their use of ML, it may still sound rather unrealistic for many EDA or design engineers when we predict ML in EDA will bring serious threats to EDA tools and softwares in the future. A common argument against ML for EDA is that many ML methods suffer from limited accuracy or unreliability, while a tiny mistake in chip design and manufacturing process can lead to chip failure. However, only simulations at sign-off stages need to be perfectly accurate, and they only account for a small portion of EDA tools in the whole design flow. Most earlier design stages accept trade-off between accuracy and runtime in tools, thus provide large rooms for ML methods. We will cover the reliability problems of ML in EDA in Section~\ref{sec:3}. 

%Our claim is based on two key observations. First, in the whole design flow, .  


\subsection{Threats or Attacking Mechanisms}

%There are two main categories of ML models. 

To better discuss the threat from ML models on EDA tools, current ML models in EDA can be categorized into two types. 
\begin{itemize}
    \item \textbf{Add-on predictive models}. Most ML models in EDA are supervised and perform prediction tasks. They are usually trained based on certain EDA tool. These models need to be used together with the target tool, either directly providing prediction results to designers, or being integrated into the flow to perform optimization based on the tool. In summary, they work as an add-on part of existing tools. 
    \item \textbf{Standalone optimization models.} Some ML models can work a standalone tool without being the part of EDA tools. They typically adopt reinforcement learning (RL) and can directly replace some functions in EDA tools. An example is the RL-based macro placer~\cite{mirhoseini2021graph} proposed by Google.    
\end{itemize}



\subsection{Defense Algorithms or Guidelines}


According to our analysis, EDA vendors should prevent unauthorised use of their tools for developing ML models, which may later become threat of these tools. However, disabling model training based on a specific software is technically very difficult, and violations of such rule cannot be easily detected by the vendor. To the best of our knowledge, this is not explicitly studied before. Here we contribute a few directions that worth exploration.


One possible defense method is to introduce watermarks to the output of EDA tools. This is possible for major design automation functions that directly modify the circuit and support multiple outputs with similar qualities, including placement, CTS, routing, and circuit optimizations at different steps. EDA vendors can design these functions to generate a tiny watermark without affecting the normal usage of the functions. The target is to have possible generative ML models learn the watermark pattern. However, it is much more difficult to generate watermarks in simulation functions where outputs are deterministic. %In addition, to make this effective, .


Another possible direction for EDA vendors is to introduce backdoor in their EDA tools. It means that for special inputs with secret triggers, the EDA tools generate unusual outputs that can be easily recognized and used as the evidence. The target is to have the backdoor learned by ML models without being perceived by model developers. If this is successful, the ML model can function properly in normal circumstance. But vendors can judge whether a model is trained on their tools by testing it with inputs with triggers. However, how to have the ML model pick up such backdoor during model construction process is a major challenge. 

%there are still major challenges to consider in this defense mechanism. 

%This backdoor has to be learned by ML models without being perceived by model developers. 


%\subsection{Experimental Results}

%We provide a simplified demonstration on inserting backdoor in EDA output and making it learned by ML models. \blue{TODO 2}



%can study defense algorithms. 




==> _txt/acknowledgement.tex <==

\section*{Acknowledgments}
This work is partially supported by Semiconductor Research Corporation Tasks 2810.021 and 2810.022 through UT Dallas’ Texas Analog Center of Excellence (TxACE).
